Modal Analysis of Spatiotemporal Data via Multivariate Gaussian Process Regression

Modal analysis has become an essential tool to understand the coherent structure of complex flows. The classical modal analysis methods, such as dynamic mode decomposition (DMD) and spectral proper orthogonal decomposition (SPOD), rely on a sufficient amount of data that is regularly sampled in time. However, often one needs to deal with sparse temporally irregular data, e.g., due to experimental measurements and simulation algorithm. To overcome the limitations of data scarcity and irregular sampling, we propose a novel modal analysis technique using multi-variate Gaussian process regression (MVGPR). We first establish the connection between MVGPR and the existing modal analysis techniques, DMD and SPOD, from a linear system identification perspective. Next, leveraging this connection, we develop a MVGPR-based modal analysis technique that addresses the aforementioned limitations. The capability of MVGPR is endowed by its judiciously designed kernel structure for correlation function, that is derived from the assumed linear dynamics. Subsequently, the proposed MVGPR method is benchmarked against DMD and SPOD on a range of examples, from academic and synthesized data to unsteady airfoil aerodynamics. The results demonstrate MVGPR as a promising alternative to classical modal analysis methods, especially in the scenario of scarce and temporally irregular data.

==> src/old/sec0_int.tex <==
\section{Introduction}

Spatiotemporal data is universally seen in aerospace and mechanical engineering applications, especially in fluid and structural dynamics.  The accurate and efficient extraction of the dominant modes and the associated with characteristic frequencies from the spatiotemporal data may contribute critically to the understanding of the underlying physical phenomena.  For example, proper orthogonal decomposition (POD) \cite{berkooz1993proper} and spectral POD \cite{schmidt2020guide, towne2018spectral} methods have been used to extract out coherent flow structures from turbulent flow; dynamic mode decomposition (DMD) \cite{schmid2011applications,kutz2016dynamic} has been employed to produce reduced-order dynamical systems representing the evolution of complex flow fields; the DMD has been further extended with the resolvent analysis techniques \cite{taira2017modal} to identify potential forcing and response modes in the flow field that may reveal potential flow mechanisms hidden in the spatiotemporal data.  Furthermore, due to its connection to the more general Koopman mode decomposition (KMD) techniques \cite{brunton2021modern}, the DMD-type techniques have enjoyed some prevalence in data-driven modal analysis of spatiotemporal data.

There are, however, still challenges associated with the existing DMD-type techniques \cite{taira2017modal,brunton2021modern,colbrook2021rigorous}. Some of the challenges include (1) Spectral pollution caused by discretization of the dynamics as well as the measurement noise, (2) Inconvenience to utilize temporally non-uniformly distributed data, due to the usual underlying assumption of uniform time step size in conventional DMD methods, and (3) Difficulty to incorporate datasets of multiple fidelities, e.g., to fuse experimental measurements with computational data consistently into a dynamical model.

To tackle the above challenges, we first note a simple fact from linear system theory \cite{Papoulis2002}. For a single-input single-output (SISO) system, if the input is Gaussian white noise, the output is a zero-mean Gaussian process (GP) with its correlation function determined by the system dynamics. Such relation extends to higher-dimensional dynamical systems \cite{sarkka2013spatiotemporal}. In other words, the identification of a linear system, of which DMD is a special case, and the estimation of a GP correlation function are equivalent.

In this work, we extend the aforementioned connection to the DMD-type models for spatiotemporal data and multi-variate Gaussian process regression (MVGPR) models \cite{Sadagopan2021a,Sadagopan2022}.  Specifically, MVGPR is shown to produce a low-order linear dynamical system for a spatiotemporal dataset; when the correlation function of MVGPR is designed properly, the model will only admit a sparse spectrum, and thus has the potential to alleviate spectral pollution.  Assuming stationarity of the MVGPR, the learning of correlation function only depends on the differences between time steps, without requiring the time step size to be uniform.  The MVGPR can be extended with a multi-fidelity component, denoted \MMG, that naturally accounts for the fusion of multi-fidelity datasets, and due to the recursive formulation of \MMG, it is possible to fuse multiple levels of fidelity.  Finally, to make the MVGPR approach more general, we establish the connection between MVGPR and Koopman operator theory, and show that MVGPR models can also learn from nonlinear dynamical data when appropriate nonlinear coordinate transformation is employed.

Building on the general-purpose \MMG framework developed previously by the authors \cite{Sadagopan2021a,Sadagopan2022}, this study aims to demonstrate the feasibility of GPR-based modal analysis of spatiotemporal data, as an alternative to DMD methods.  Specifically, the goals of this paper are to
\begin{enumerate}
    \item Present the theoretical formulation of \MMG for modal analysis of spatiotemporal data.
    \item Reveal the connections among \MMG, linear system identification, and Koopman analysis.
    \item Benchmark the single-fidelity portion of \MMG against DMD on multiple problems to highlight its robustness in the presence of noisy data and incomplete data.
\end{enumerate}

% Gaussian process is a collection of random variables which forms a joint Gaussian distribution over the variables. It is often called non-parametric Bayesian inference technique due to its two main features. First, GP computes the posterior distribution using the prior information about the types of functions, e.g., smooth or periodic functions. Second, unlike conventional linear regression which is a parametric approach, GP is non-parametric in a sense that the size of model and hence the prediction process grows with the size of the training data set. These features lead to the specification of prior because it determines the properties of functions considered in the inference \cite{williams2006gaussian}, which may include smoothness, periodicity, or other features of the function, and they are induced by so-called covariance function. In addition, the non-parametric feature of GP also allows us to analyze the model with sparse data points which will be discussed later. However, when the data is high dimensional where each of them are correlated to one another, the traditional GP is not able to capture this correlation. 

% To handle this issue, multi-variate GPR is used to analyze the information across the output space \cite{futoma2017learning}. If this correlation is not considered in the modeling, the result is nothing but the simple combination of uni-variate GPR. There are many types of models that handles this feature. The Intrinsic Coregionalization Model (ICM) \cite{babak2007comparison} is the most simplistic form of multi-variate GP in which each output shares the same latent structure. On the other hand, Linear Coregionalization Model (LMC) takes into account the different latent structures existing in the dynamical system. In this paper, we demonstrate that Multi-fieldity Multi-output GPR (M2GPR) has a capability to overcome both challenges by considering cylinder vortex flow.

==> src/old/sec1_pre.tex <==
\section{Preliminaries}
This section presents a brief summary of the Koopman analysis framework and the standard DMD technique, as a basis for the development of new methodology.

\subsection{Koopman Mode Analysis}
In this study, we are interested in autonomous nonlinear dynamics of the following form,
\begin{equation}
    \dot\vx = \vf(\vx),\quad \vx(0)=\vx_0
\end{equation}

From an operator theoretic point of view \cite{brunton2021modern,mezic2013analysis}, there exists a mapping of the finite dimensional states $\vx$ to a functional $g(\vx)$, called observable, in an infinite dimensional space, so that the functional evolves linearly in time with the (continuous-time) Koopman operator,
\begin{equation}
    \dot g = \mathcal{K} g
\end{equation}
For nonlinear dynamics in the attraction basin of equilibrium points and periodic orbits, e.g., limit cycles, one can identify a finite set of pairs of eigenvalues $\lambda_i=\zeta_i+i\omega_i$ and eigenfunctions $\phi_i(\vx)$, such that
\begin{equation}
    \mathcal{K}\phi_i = \lambda_i\phi_i
\end{equation}
The set of eigenpairs form an invariant space, and if an observable $g_j$ can be decomposed in terms of the eigenfunctions,
\begin{equation}
    g_j(\vx) = \sum_{i=1}^N \phi_i(\vx) \langle \phi_i(\vx), g_j(\vx) \rangle
\end{equation}
where $\langle\cdot,\cdot\rangle$ indicates inner product, then the dynamical response of the observable can be represented by a finite-dimensional series
\begin{equation}
    g_j(t) = \sum_{i=1}^N \exp(\lambda_i t)\phi_i(\vx_0) \langle \phi_i(\vx_0), g_j(\vx_0) \rangle \equiv \sum_{i=1}^N \exp(\lambda_i t)\Gamma_{ij}
\end{equation}
Suppose there are multiple observables, $\vg=[g_1,g_2,\cdots,g_M]^T$,
\begin{equation}\label{eqn_obs_dyn}
    \vg(t) = \sum_{i=1}^N \exp(\lambda_i t) \vtg_i \equiv \vtG\exp(\vtL t)
\end{equation}
where $\vtg_i=[\Gamma_{i1},\Gamma_{i1},\cdots,\Gamma_{iM}]^T$ represents a dynamic mode in $\vg$ that evolves with eigenvalue $\lambda_i$, i.e., with frequency $\omega_i$ and damping $\zeta_i$.

\subsection{Modal Analysis by DMD}
Dynamic Mode Decomposition (DMD) is a standard method for extracting dynamically relevant modes, or arguably the Koopman modes, from a dataset of trajectories.  Consider just one trajectory $\cD=\{(t_i,\vx_i)\}_{i=1}^n$, sampled uniformly with time step size $\Delta t$, one may form data matrices $\mathbf{X}, \mathbf{X}^{'} \in \mathbb{R}^{m \times (n-1)}$ with observables $\vg$,
\begin{equation}\label{data_matrix}
    \mathbf{X} = \begin{bmatrix}
    \vg(\mathbf{x}_1) & \vg(\mathbf{x}_2) & \cdots & \vg(\mathbf{x}_{n-1})
    \end{bmatrix}, \quad \mathbf{X}' = \begin{bmatrix}
    \vg(\mathbf{x}_2) & \vg(\mathbf{x}_3) & \cdots & \vg(\mathbf{x}_n)
    \end{bmatrix}
\end{equation}
The DMD effectively produces a finite-dimensional discrete-time approximation $\vA$ of the Koopman operator, such that $\vX'=\vA\vX$; standard least squares gives $\vA=\vX'\vX^+$, where $\Box^+$ is pseudo-inverse.  For practical calculations where the dimension of $\vg$ is high, it is typical to approximate the pseudo-inverse by a truncated SVD,
\begin{equation}
    \mathbf{X} = \mathbf{U}\mathbf{\Sigma} \mathbf{V}^{*} \approx \mathbf{U}_r \mathbf{\Sigma}_r \mathbf{V}_r^{*} \Rightarrow \vX^+=\vV_r\vtS_r\vU_r^*
\end{equation}
where $\Box^*$ indicates conjugate transpose and $r$ a reduced dimension.  Next, via the eigendecomposition of a projected $\vA$,
\begin{equation}
    \bar{\vA} \equiv \vU^{*}_r\vX'\vV_r\vtS_r^{-1} = \vW\bar{\vtL}\vS^*
\end{equation}
one can recover the eigenpairs of $\vA$, i.e., the approximate Koopman modes and Koopman eigenvalues,
\begin{equation}
    \vtG = \vU_r\vW,\quad \vtL = \log(\bar{\vtL})/\Delta t
\end{equation}

There are two potential issues, among the others, with the DMD approach \cite{colbrook2021rigorous}.  One issue is data noise, which would significantly impact the quality of the truncated SVD and thus the identified Koopman eigenpairs.  A typical technique is to employ an ensemble technique to average out DMD results over many noisy trajectories, yet such approach relies on the availability of a large high quality dataset that is often unavailable \cite{duke2012error}.  Another issue is the missing data, such that the data samples are not uniformly distributed over time.  This issue might completely overthrow the DMD formulation.  One remedy is to employ an optimization-based formulation to directly learn the continuous-time operator, the computational complexity of which, however, is high \cite{askham2018variable}.

% where $\mathbf{A} \in \mathbb{R}^{m \times m}$ is best-fit approximated linear operator that maps a snapshot at a particular time step to the state at the next time step. The dynamic mode is referred to as the eigenvector of the matrix $\mathbf{A}$.

% \begin{equation}\label{dynamic_op}
%     \mathbf{X}^{'} = \mathbf{A}\mathbf{X}, \quad \mathbf{A} = \mathbf{X}^{'}\mathbf{X}^{*}
% \end{equation}

% Typically, if the size of the state, $m$ is large, then it is computationally intractable to analyze the eigenvalues and eigenvectors directly. However, one can avoid this computation by making use of the modes projected on the POD space.
% \begin{equation}
%     \mathbf{X} = \mathbf{U}\mathbf{\Sigma} \mathbf{V}^{*}, \quad \mathbf{X} \approx \mathbf{U}_r \mathbf{\Sigma}_r \mathbf{V}_r^{*}
% \end{equation}

% The second equation in Eq. (\ref{dynamic_op}) can be represented using the POD bases as shown in Eq. (\ref{low_dynamic_op}). 
% \begin{equation}\label{low_dynamic_op}
%     \mathbf{A} = \mathbf{X}^{'}\mathbf{V}_r\mathbf{\Sigma}_r^{-1}\mathbf{U}_r^{*}
% \end{equation}

% The low-dimensional matrix $\tilde{\mathbf{A}}$ can be obtained by projecting $\mathbf{A}$ on the POD bases.
% \begin{equation}\label{dmd_low_eig}
%     \tilde{\mathbf{A}} = \mathbf{U}_r^{*}\mathbf{A}\mathbf{U}_r = \mathbf{U}_r^{*}\mathbf{X}^{'}\mathbf{V}_r\mathbf{\Sigma}_r^{-1}
% \end{equation}

% The real and imaginary part of the eigenvalue of $\tilde{\mathbf{A}}$ which is denoted as $\tilde{\mathbf{\Lambda}}$ in Eq. (\ref{dmd_low_eig}) represents the damping and frequency of corresponding mode respectively.

% \begin{equation}
%     \tilde{\mathbf{A}}\mathbf{W} = \mathbf{W}\tilde{\mathbf{\Lambda}}
% \end{equation}

% If we project this back to the original space, then the eigenvalue and eigenvector of $\mathbf{A}$ is given by $\mathbf{\Lambda}$ and $\mathbf{U}_r \mathbf{W}$ respectively. The $\mathbf{U}_r\mathbf{W}$ is called \textit{projected DMD}.

% \begin{equation}
%     \mathbf{A}\mathbf{U}_r\mathbf{W}= \mathbf{U}_r\mathbf{W}\mathbf{\Lambda}
% \end{equation}

==> src/old/sec2_gpr.tex <==
\section{System Identification using Gaussian Processes}
This section presents the formulation of \MMG, the spectral representation of linear system models, and their connections.  Based on these connections the \MMG is posed as an alternative approach to the Koopman modal analysis of nonlinear dynamics.

\subsection{Multi-fidelity Multivariate Gaussian Process Models}
In the context of dynamical systems, \MMG is defined over a single input, time; for the general case of multi-dimensional inputs, see Ref. \cite{Sadagopan2021a}.

\subsubsection{Single-Fidelity Univariate GPR}
To establish the terminology, we start with the relatively simple univariate version of GPR (UVGPR), which only returns one output, and only consider dataset of one fidelity level. The univariate GPR model is based on the following Gaussian process model \cite{Rasmussen2006,Forrester2008},
\begin{equation}
  x_{UV}\sim \GP(m(t),k(t,t'))
\end{equation}
where $m(t)$ is a scalar mean function that captures the global trend in the data and $k(t,t')$ is a scalar correlation function to account for the deviation of the data from the global trend.  A non-zero mean function may be useful for capturing transient dynamics for flows in non-equilibrium, but for statistically converged unsteady flows we assume $m(t)=0$ and $k(t,t')=k(t-t')\equiv k(\tau)$. This assumption will be employed in the following.

Given a dataset $\cD=\{(t^{(i)},\vx^{(i)})\}_{i=1}^{N_s}$ of vector output, one UVGPR $x_{UV,j}$ is generated for the $j$th output; and for a new input $t^*$ the prediction is given by the Gaussian distribution,
%\begin{equation}\label{eqn_s2gpr}
  $x_{UV,j}(t^*)\sim \cN(\mu(t^*;\cD),\sigma^2(t^*;\cD))$,
%\end{equation}
with the mean $\mu$ providing the prediction and variance $\sigma^2$ providing the error estimate.  The detailed expressions of $\mu$ and $\sigma^2$ are available in Refs. \cite{Rasmussen2006, Forrester2008}.

%----------------------------------------------------------------------------------
\subsubsection{Single-Fidelity Multivariate GPR}
For cases where multiple outputs are involved, while it is possible to train one UVGPR for the prediction of each output, a more efficient approach is to employ a multivariable GPR (MVGPR) formulation.  The MVGPR also accounts for the correlation between the outputs and arguably provides higher accuracy than its univariate counterpart.  The MVGPR relies on a multivariate GP,
\begin{equation}
  \vx_{MV}\sim \GP(0,\vK(t,t'))
\end{equation}
where $\vK(t,t')$ is a matrix of $N_y\times N_y$ correlation functions.  The $(i,j)$th element of $\vK$ indicate the correlation between the $i$th and $j$th outputs.  Similar to the univariate case, the prediction at a new input $t^*$ is represented using a multivariate Gaussian distribution; see Refs. \cite{Parussini2017,Sadagopan2021a,Sadagopan2022} for details.

To guarantee the well-posedness of the MVGPR model, the correlation function needs to be chosen carefully.  One possibility is the linear model of coregionalization (LMC).  A rank-$N_K$ LMC model is a weighted sum of $N_K$ scalar correlation functions $\{k_j(t,t')\}_{j=1}^{N_K}$ \cite{Alvarez2012,Parussini2017},
\begin{equation}\label{eqn_lmc}
    \vK(t,t')=\vtG[\mathrm{diag}(k_1,k_2,\cdots,k_{N_K})]\vtG^T=\sum_{j=1}^{N_K}\vtg_j\vtg_j^T k_j(t,t')
\end{equation}
where the weight matrix $\vtG$ is of size $N_y\times N_K$, and its column vector $\vtg_j$ represents the correlation between the outputs and has to be estimated during the training of the MVGPR.  The $N_y$ scalar correlation functions can be different or partially same.  One can choose either $N_K<N_y$ to reduce the number of parameters in the matrix correlation function, or $N_K\geq N_y$ to capture complex correlations between the outputs.

The MVGPR with the LMC kernel in Eq. (\ref{eqn_lmc}) is equivalent to the linear combination of $N_K$ independent UVGPR's,
\begin{equation}\label{eqn_mv_uv}
  \vx_{MV}(t) = \vtG\vg_{UV}(t)
\end{equation}
where $g_{UV,i} \sim \GP(0,k_i(t,t'))$.  This relation also shows that, if the correlation between the outputs is ignored, i.e., if $\vtG$ is a $N_y\times N_y$ identity matrix, the MVGPR reduces to $N_y$ UVGPR's, where the UVGPR models are generated for each of the outputs independently.

It is also noteworthy that Eq. \eqref{eqn_mv_uv} also performs a dimensionality reduction of high-dimensional output data, where the columns of the weight matrix $\vtG$ are effectively the dominant modes of the data.  The MVGPR identifies the dominant modes and generates the mapping from input to modal coordinates \textit{simultaneously}.  The MVGPR modes are different from the modes obtained in standard methods, e.g., POD or principle component analysis (PCA), because the latter does not account for the distribution of inputs.

%-------------------------------------------------------------------------------
\subsubsection{Multi-Fidelity Multivariate GPR}
Lastly we augment the MVGPR formulation to account for datasets of multiple fidelity levels.
Usually the data of higher fidelity is more expensive to generate and hence more sparse in the parameter space.  The multi-fidelity GPR formulation provides a natural way to fuse the datasets.  In the following, we consider a low-fidelity (LF) dataset $\cD_{LF}=\{(t_{LF}^{(i)},\vx_{LF}^{(i)})\}_{i=1}^{N_{LF}}$ and a high-fidelity (HF) dataset $\cD_{HF}=\{(t_{HF}^{(i)},\vx_{HF}^{(i)})\}_{i=1}^{N_{HF}}$.

The data assimilation is achieved using the level-1 auto-regressive approach \cite{Brevault2020}, which is applicable to datasets of multiple levels of fidelity.  To maintain the relevance with the context of this paper, we keep the discussion for the case of two fidelity levels.
A multivariate GP of the following form is introduced
\begin{equation}
  \vx_{HF} = \vtr(t)\odot \vx_{LF}(t) + \vtd(t)
\end{equation}
where $\vx_{LF}\sim\GP(0,\vK_{LF}(t,t'))$ and $\vtd(t)\sim\GP(0,\vK_{\delta}(t,t'))$ are GP's for the LF dataset and the difference between the LF and HF datasets, respectively,
$\vtr(t)$ is a vector-valued scaling factor to tune the contribution of the $\vx_{LF}(t)$, and $\odot$ means element-wise product.

For the multi-fidelity formulation, it is assumed that the GP's $\vtd(t)$ and $\vx_{LF}(t)$ are independent, so that no more information is present in the LF dataset when compared to the HF dataset.  Therefore, a two-stage procedure is employed to train the multi-fidelity GPR.  First, the GP $\vx_{LF}(t)$ is trained as if a MVGPR using the LF dataset $\cD_{LF}$.  Next, the scaling factor $\vtr(t)$ combined with the LF component is treated as a composite mean function, and the GP $\vx_{HF}(t)$ is trained again as a MVGPR using the HF dataset $\cD_{HF}$.  Eventually, the multi-fidelity prediction $\vx_{MF}$ given a new input $t^*$ is based on a new Gaussian distribution \cite{Sadagopan2021a,Sadagopan2022}.

Once the LF and HF datasets are available, one can use a \textit{full \MMG} approach to connect the input vector $t$ to the high-dimensional output $\vx$.
\begin{equation}
  \vx(t) = \vx_{MF}(t) = \vtr(t)\odot\vtG_{LF}\vg_{UV,LF}(t) + \vtG_{\delta}\vg_{UV,\delta}(t)
\end{equation}
where the $\vtG_{LF}$ and $\vtG_{\delta}$ represent the dominant patterns in the LF dataset and the difference between the LF and HF datasets.  When compared to the MVGPR formulation, the \MMG approach provides even higher flexibility to characterize the HF data distribution, especially when the LF model approximates the HF model well.


%----------------------------------------------------------------------------------
\subsection{Conversion Between Gaussian Processes and MIMO Linear Systems}

%----------------------------------------------------------------------------------
\subsubsection{Linear Time-Invariant System}
First we examine a basic example that connects a UVGPR to a SISO system. Consider an $n$-th order linear time-invariant (LTI) system,
\begin{equation}\label{eqn_lti}
\frac{d^n f(t)}{d t^n} + a_{n-1}\frac{d^{n-1} f(t)}{d t^{n-1}} + ... + a_{1} \frac{d f(t)}{d t} + a_0 f(t) = w(t)
\end{equation}
where $w(t)$ is a Gaussian white noise with zero mean whose spectral density $S_w(\omega) = q_c$. The response $f(t)$, therefore, is a GP with zero mean.  The correlation function $k(\tau)$ of $f(t)$ can be identified using the Wiener-Khinchin theorem via its spectral density $S(\omega)$.  Specifically, from the Fourier transform of Eq. \eqref{eqn_lti},
\begin{equation}
    S(\omega) = \norm{G(i\omega)}^2q_c,\quad G(i\omega)=\frac{1}{(i \omega)^n + a_{n-1}(i \omega)^{n-1} + \cdots + a_{1} (i \omega) + a_0}
\end{equation}
where $G(i\omega)$ is the transfer function.  Subsequently, the correlation function is found by inverse Fourier transform
\begin{equation}
k(\tau) = \cF^{-1}[S(\omega)] = \int_{-\infty}^{\infty}{S(\omega)\exp\left( i\omega \tau \right)} d \omega
\end{equation}

Conversely, if one obtains the correlation function $k(\tau)$, e.g., from the Gaussian process regression of a LTI system response, $k(\tau)$ may be leveraged to obtain the spectral density $S(\omega)$ and then reconstruct at least the stable component of the linear system, based on the classical control theory; this is the spectral factorization process \cite{Papoulis2002,sarkka2013spatiotemporal}.

\subsubsection{Tackling Harmonic Responses}

Nevertheless, the spectral factorization cannot be applied to periodic functions and its covariance, since the rational form of spectral density cannot approximate that of periodic functions \cite{solin2014explicit}.
As a motivating example, consider a coupled harmonic oscillator at frequency $j\omega_0$
\begin{equation}\label{eqn_cho}
\left\{
    \begin{array}{l}
      \ddt{x_j(t)} = -j \omega_0 y_j(t) \\
      \ddt{y_j(t)} = j \omega_0 x_j(t)
    \end{array}
\right.
\end{equation}
whose solution is
\begin{equation}
\label{}
\bold{x}_j(t) = 
\begin{bmatrix}
\cos(j\omega_0 t ) & -\sin(j\omega_0 t) \\
\sin(j\omega_0 t)  & \cos(j\omega_0 t)
\end{bmatrix}\bold{x}_j(0)
\end{equation}
where $\bold{x}_j(0) \sim \cN(0, q_j^2\vI)$. The covariance function of the response is retrieved by calculating $\mathop{\mathbb{E}}(x_j(t) x_j(t + \tau))$.  This process produces a Cosine kernel $k_p(\tau)$ for $x_j$, whose spectral density $S_p(\omega)$ contains Dirac delta functions,
\begin{align}\label{eqn_kpt}
k_p(\tau) &= {q_j^2\cos(j\omega_0\tau)} \\\label{eqn_spw}
S_p(\omega) &= {q_j^2 \pi [\delta(\omega - j \omega_0) + \delta(\omega + j \omega_0)]}
\end{align}
The Dirac delta functions cannot be well approximated using rational functions, and pose a challenge in the spectral factorization process.

Nevertheless, leveraging GP, the spectral factorization can be bypassed and one can directly establish the mapping between a specific covariance function and a specific linear system.  For example, one may assume a Cosine kernel Eq. (\ref{eqn_kpt}) for GP, learn the parameter $j\omega_0$ from data, and infer that the observed dynamics is governed by the linear system Eq. (\ref{eqn_cho}).

Similarly, if one employs the Mat\'ern kernel family,
\begin{equation}
\label{matern}
k_\nu(\tau) = \sigma^2 \frac{2^{1- \nu}}{\Gamma(\nu)}\left(\sqrt{2 \nu} \frac{\tau}{l}\right)^{\nu} K_{\nu}\left(\sqrt{2\nu}\frac{\tau}{l}\right)
\end{equation}
or more specifically when $\nu=1/2$,
\begin{equation}
    k_{1/2}(\tau) = \sigma^2 \exp{\left(-\frac{\tau}{l}\right)}
\end{equation}
the resulting GP with a Mat\'ern-12 kernel corresponds to an exponentially decaying system with a decay rate of $1/l$ \cite{sarkka2013spatiotemporal}.  Furthermore, the combination of Mat\'ern-12 and Cosine (MC) kernels
\begin{equation}\label{eqn_kmc}
    k_{MC}(\tau) = \sigma^2\exp{\left(-\frac{\tau}{l}\right)}\cos(\omega\tau)
\end{equation}
produce a damped oscillation response \cite{solin2014explicit}.  The MC kernel reduces to Mat\'ern-12 and Cosine when $\omega\rightarrow 0$ and $l\rightarrow\infty$, respectively.

\subsubsection{The Multivariate Case}
Subsequently, the previous formulation for systems with a single output can be extended to those with multiple outputs.  Consider a linear system with i.i.d. Gaussian white noise inputs $\vu\sim\cN(0,\sigma^2\vI)$,
\begin{equation}
    \dot{\vx} = \vA\vx + \vB\vu
\end{equation}
Apparently $\vx$ follows a Gaussian process with zero mean and a certain correlation function $\vK(\tau)$ that depends on $\vA$ and $\vB$.  Note that $\vA$ is given by system dynamics and fixed, but the choice of $\vB$ is arbitrary.

Assuming an eigendecomposition $\vA=\vtF\vtL\vtY^*$ exists, the system gain matrix is
\begin{equation}
    \vG(i\omega) = (i\omega\vI-\vA)^{-1}\vB = \vtF(i\omega\vI-\vtL)^{-1}\vtY^*\vB
\end{equation}
and the spectral density of the states is
\begin{equation}
    \vS(\omega) \propto \vG(i\omega)\vG(i\omega)^* = \vtF(i\omega\vI-\vtL)^{-1}\vtX(i\omega\vI-\vtL)^{-1}\vtF^*
\end{equation}
where $\vtX=\vtY^*\vB\vB^*\vtY$.  Suppose $\vB=\vtF$, then $\vtX=\vI$, and
\begin{equation}\label{eqn_msf}
    \vS(\omega) \propto \vtF(i\omega\vI-\vtL)^{-2}\vtF^* \Rightarrow \vK(\tau) \propto \vtF\cF^{-1}\left[(i\omega\vI-\vtL)^{-2}\right]\vtF^*
\end{equation}
where the portion of inverse Fourier transform in $\vK(\tau)$ is clearly diagonal, making it in the form of an LMC kernel.

Conversely, one can bake in an \textit{inductive bias} into a MVGPR model using an LMC kernel with weight matrix $\vtG$ and appropriate kernels $\{k_i\}_{i=1}^{N_K}$.  Such functional form enforces the model to learn a correlation function in the form of Eq. (\ref{eqn_msf}).  In this case, $\vtG$ coincides with eigenvectors of $\vA$, which are the Koopman eigenvectors of the underlying nonlinear system, and the kernel parameters shall reveal the Koopman eigenvalues.

\subsubsection{Gaussian Process for Modal Analysis}
Hitherto, the connections among MVGPR, linear systems, and Koopman analysis have been established.  Basically, training a MVGPR with an appropriate LMC kernel on a dataset of trajectories is shown to reveal the Koopman modes and eigenvalues of the nonlinear dynamics.

Given a dataset of trajectories $\cD=\{(t_i,\vx_i)\}_{i=1}^N$, the algorithm for modal analysis based on MVGPR is formalized as follows,
\begin{enumerate}
    \item If the $\vx$'s are of very high dimension, it would be beneficial to project the data onto a reduced space, producing a new dataset $\hat{\cD}=\{(t_i,\hat{\vx}_i)\}_{i=1}^N$ where $\hat{\vx}=\vP\vx$.  The projector $\vP$ can be found by, e.g., standard POD procedure.
    \item Select appropriate observables $\vg$ following standard guidelines of DMD method.
    \item Determine the number of modes of interest, and select the kernel for each potential Koopman mode.  For simplicity one can choose the MC kernel Eq. (\ref{eqn_kmc}) and let the learning process decide the kernel parameters.
    \item Learn the MVGPR from data using a GP implementation, and the LMC kernel produces weight matrix $\vtG$ and other kernel parameters such as decay rate and frequency.
    \item The Koopman modes are recovered by $\vP^+\vtG$ and the Koopman eigenvalues are recovered by other kernel parameters.
\end{enumerate}

% Consider following linear state-space model with i.i.d. white noise input $\vu\sim\cN(0,\sigma^2\vI)$, where the $j$th entry is the zero-mean Gaussian distribution with standard deviation $\sigma$, $u_j \sim N(0, \sigma^2)$.
% \begin{equation}\begin{split}
%     \dot{\vx} &= \mathbf{A} \mathbf{x} + \mathbf{u} \\
%     \vy &= \mathbf{U}_r\mathbf{x}
% \end{split}
% \end{equation}
% where $\mathbf{U}_r$ is the POD modes.
% Now, consider the same linear system mapped onto the eigenvector space as shown in Eq. (\ref{eigensys}). 

% \begin{equation}\begin{split}\label{eigensys}
%     \dot{\vz} &= \tilde{\mathbf{\Lambda}} \mathbf{z} + \mathbf{S}^{*}\mathbf{u} \\
%     \mathbf{y} &= \mathbf{U}_r\mathbf{W}\mathbf{z}
% \end{split}
% \end{equation}
% where $\mathbf{z} = \mathbf{S^*}\mathbf{x}$ and $\mathbf{A} = \mathbf{W}\tilde{\mathbf{\Lambda}}\mathbf{S}^*$ where $\mathbf{W}$ and $\mathbf{S}$ are right and left eigenvectors, and $\tilde{\mathbf{\Lambda}}$ is diagonal eigenvalue matrix. In this representation, the components of the noise are weighted by the left eigenvector, $\mathbf{S}$. In the first equation of Eq. (\ref{eigensys}), each $z_{j}$ is zero mean independent Gaussian process, $ z_{j} \sim \GP(0, k_{z_jz_j})$. Therefore, the cross covariance between $z_i$ and $z_j$ is zero when $i \neq j$.

% \begin{equation}\label{kernstruct}
% \mathbf{K}_{\mathbf{yy}} = \left(\mathbf{U}_r\mathbf{W}\right)\mathbf{K}_{\mathbf{zz}}\left(\mathbf{U}_r\mathbf{W}\right)^{*}
% \end{equation}

% If $\mathbf{U}_r\mathbf{W}$ is replaced by $\mathbf{B}$, one can find that the specific form of Eq. (\ref{kernstruct}) is same as Eq. (\ref{eqn_lmc}) which was explained in the context of LMC. By this representation, the modes can be obtained by $\mathbf{U}_r\mathbf{W}$.

==> src/old/sec3_res.tex <==
\section{Results and Discussion}
This section demonstrates the mode decomposition methodology using the single-fidelity portion of \MMG using a range of examples.  First, results are presented for two academic problems to illustrate the workings of the MVGPR method.  Second, the MVGPR method is applied to more realistic flow field datasets and benchmarked against DMD to highlight the unique advantages of MVGPR.

\subsection{Problem 1: Spatiotemporal Stationary Waves}
The first problem is a linear combination of stationary waves, to illustrate the capability of MVGPR to extract out modes and frequencies robustly in the presence of noise.  Note that the stationary waves pose an extra challenge to standard DMD approach and requires extension to, e.g., higher-order DMD methods for the correct identification of modes \cite{tu2013dynamic}.

The spatiotemporal data is defined as follows,
\begin{equation}\label{eqn_st_dat}
    \vx(s,t) = \sum_{i=1}^6 exp(-t/l_i)\cos(f_i t+\varphi_i) M_i(s) + \epsilon(s,t)
\end{equation}
where $s$ is the spatial coordinate, the frequencies $f_i$ and decay rates $1/l_i$ are listed in Table \ref{tab:st}, and $M_i$ are spatial modes,
\begin{equation}
\begin{aligned} 
M_1(s) = e^{-2 s^2}\cos{(2 \pi s)},\quad M_2(s) = e^{-2(s-0.5)^2},\quad M_3(s) = \frac{1}{1+9s^2} \\
M_4(s) = e^{-2s} \cos(6 \pi s),\quad M_5(s) = M_4^2(s),\quad M_6(s) = M_4^3(s)
\end{aligned}
\end{equation}
Gaussian white noise $\epsilon$ with variance $\sigma$ is added to Eq. \eqref{eqn_st_dat}, and two cases are considered: (1) Low noise with $\sigma=10^{-4}$ and (2) High noise with $\sigma=10^{-1}$.  In MVGPR modeling, 6 MC kernels and 1 squared exponential kernel are used to capture the 6 modes and the white noise, respectively.

The spatial coordinates are sampled uniformly over $[0,2]$, and the time is sampled with a step size 0.02s over $[0,10]$ seconds.  The phase angles $\varphi_i$ are randomized to generate multiple trajectories; two trajectories are used for each case.  The trajectories from 0-5 secs are used for training and 5-10 secs for testing.

% To account for different trajectories, 
% one-hot encoding along with the automatic relevance determination (ARD). 
% To be specific, each set of trajectory is labeled in the data set, and one squared exponential kernel is multiplied to the kernel set. 
% This kernel now learns the correlation between the trajectories. 
% Thus, when properly learned, the lengthscale of the kernel represents the degree of correlation.

The time-domain predictions are shown in Fig. \ref{st_time}, where the MVGPR responses and true responses are compared at several spatial locations, with $\pm$1 standard deviation.  In both cases, the mean of MVGPR matches well with the true response, while the standard deviation bounds characterize the noise level correctly.  Furthermore, the modes and eigenvalues identified from both cases are shown in Fig. \ref{mode_comparison} and Table \ref{tab:st}, respectively.  The MVGPR predictions match well with the true data, especially for the second case despite the high noise level.

\begin{table}[H]
\caption{\label{tab:st} Parameters relevant to the linear spatiotemporal data}
\centering
\begin{tabular}{p{3cm}cccccc}
\hline
$(f, l^{-1})$ & $M_1$ & $M_2$ & $M_3$ & $M_4$ & $M_5$ & $M_6$\\
\hline
True  & (1.0, 1.2) & (3.0, 5.3) & (5.2, 10.1) & (3.6, 12.1) & (7.6, 7.6) & (3.3, 2.6)\\
Low noise & (0.96, 1.27) & (2.99, 5.1) & (5.19, 10.0) & (3.59, 11.6) &(7.59, 7.91) & (3.26, 2.41) \\ 
High noise & (1.02, 1.29) & (2.99, 5.2) & (5.2, 10.3) & (3.6, 12.4) & (7.6, 7.9) & (3.29, 2.92) \\
% \% error (low noise) & (4.0\%, 5.9\%) &(0.46\%, 3.8\%) &(0.15\%, 0.04\%) &(0.2\%, 1.35\%) &(0.07\%, 4.1\%) &(1.1\%, 7.48\%) \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[hbt!]
\centering
\insertfigs{st_1e4_time}{0.48}{Low noise with $\sigma=10^{-4}$.}
\insertfigs{st_1e1_time}{0.48}{High noise with $\sigma=10^{-1}$.}
\caption{The MVGPR prediction vs true response at three different spatial locations.}
\label{st_time}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[width=.9\textwidth]{mode_comparison}
\caption{Comparison between true and identified modes}\label{mode_comparison}
\end{figure}




\subsection{Problem 2: Nonlinear Oscillator}
The second problem is the Van der Pol (VdP) oscillator, a well-known system having limit cycles, to demonstrate the validity of the nonlinear extension of the MVGPR approach.
Theoretically, the VdP oscillator contains infinite number of peaks in the frequency spectrum; however, for a finite dimensional approximation, it is sufficient to truncate the system for the lowest few frequency peaks.  To faciliate the Koopman formulation, polynomial basis upto 7th power is used to construct the observables.  Subsequently, 30 Cosine kernels are used in MVGPR to capture the time correlation.

The trajectory is collected from 0 to 50 seconds and to have the response at the limit cycle, initial transient response is ignored. Data collected from 40 to 50 seconds is used for test.
In Fig. \ref{unit_circle}, the results from GPR and eDMD are shown. For eDMD, we can obtain the eigenvalues that comprise the LCO; other spurious eigenvalues are identified and removed via residual-based filtering \cite{colbrook2021rigorous}. For GPR, the frequencies are comparable to the ones identified by eDMD. One can clearly see that the dominant frequencies are captured well by GPR model.  Fig. \ref{unit_circle} also illustrates an interesting difference between eDMD and GPR. In eDMD the pruning of spectrum happens \textit{a posteriori}; in GPR there is an inductive bias due to the kernel structure which effectively prunes the spectrum \textit{a priori}. In Fig. \ref{vanderPol_obser_gp}, the time-domain dynamics are learned by GPR model. The general oscillatory behavior is captured, but there exists a slight level of discrepancy between the truth and GPR mean, which is due to the bias of the posterior GPR distribution.

% Note that given the Cosine kernels the MVGPR effectively approximates the limit cycle with a set of Fourier modes, and due to the non-smooth jumps in the first VdP state, the Fourier approximation of MVGPR shows some mild high-frequency oscillations.  This problem can be alleviated using more Cosine kernels, or be eliminated using enhanced nonlinear observables.

\insertfigr{unit_circle}{0.4}{Comparison of power spectral densities of the states.}
\insertfigr{vanderPol_obser_gp}{0.57}{Comparison of GPR prediction and true response of van der Pol oscillator.}

\subsection{Problem 3: Cylinder Flow}
The third and last problem provides a more challenging test and benchmark of the MVGPR approach to highlight its robustness in noisy data and missing data.  The baseline data is the cylinder flow field in limit cycle oscillation, that is publicly available \cite{kutz2016dynamic}. The spatial dimensions of data are $199 \times 449$, and there are 151 time steps with the data sampling frequency of 1/3Hz, which gives uniform time steps from 0 to 5 seconds.

\subsubsection{Noisy Measurement Data}
In this test case, spatiotemporal noise is added to the clean flow field data $\vx(t) \in \bR^m$,
\begin{equation}
    \tilde{\vx}(t) = \vx(t) + \sum_{j=1}^{n} \vty_j c_j(t)
\end{equation}
where the noise is added via a set of spatiotemporal modes.  The noisy spatial modes $\vty_j\sim\cN(0,\sigma_1^2\vI_m)$ are sampled once and fixed; the temporal coordinates $c_j(t)\sim\GP(0,\sigma_2^2\delta(\tau))$ are sampled multiple times if multiple trajectories are desired.  In this section, $\sigma_1$ is always fixed to be $1$, and $\sigma_2$ is varied to see the effect of noise; two noisy modes are added.

% In this section, we will demonstrate the robustness of GPR when noisy measurement is given, especially for the noise associated with both spatial and temporal dimension. Consider following form of noisy measurement

% \begin{equation}
%     \tilde{\mathbf{X}} = \mathbf{X} + \sum_{i=1}^{n} \boldsymbol{\psi}_i\mathbf{c}^{T}_i
% \end{equation}
% where $\mathbf{X}$ is the original spatiotemporal data matrix, $\mathbf{c}_i \in \mathbb{R}^{n}$ is the noise associated with temporal dimension, and $\boldsymbol{\psi}_i \in \mathbb{R}^{m}$ is the noise associated with spatial dimension, $\mathbf{c}_i \sim N(0, \sigma_1^2\mathbf{I}_n), \; \boldsymbol{\psi}_i \sim N(0, \sigma_2^2\mathbf{I}_m)$.
% In this section, $\sigma_1$ is always fixed to be $1$, and only $\sigma_2$ is varied to see the effect of noise.

To facilitate efficient training of GPR, the noisy dataset is projected onto a lower-dimensional space using POD prior to the training. The POD truncation is intentionally conservative and retains more POD modes than the number of dynamic modes of interest.  The extra POD modes are involved to enrich the subspace from which the dynamic modes will be constructed.  Specifically, for GPR model, we employed 9 kernels, 8 Cosine kernels and 1 white kernel, with 14 POD modes. Every two cosine kernels correspond to one frequency component, i.e., the real and imaginary parts of the dynamic mode.

In Fig. \ref{fig:dmd_gpr_freq}, identified frequencies from DMD and GPR are displayed along with the frequencies from the DMD without noise. Both frequencies from DMD and GPR match with the DMD without noise. Since the spectrum of white noise is distributed throughout the entire frequency domain, DMD can still extract harmonic frequencies no matter how noisy the data is.

In Fig. \ref{fig:gp_temporal}, the POD coordinates with noise used to train the GPR model is compared with the true noise-free trajectories, the GPR mean prediction, and GPR error bounds given by standard deviation. It is shown that the GPR mean aligns well with the true POD coordinates and the error bound captures the fluctuation of noise well.

The mode shapes computed by GP and DMD are shown in Fig. \ref{fig:dmd_gp_modes}. The identified modes from GPR is almost same as the true DMD modes for $\sigma_2=0.5$ while this level of noise already effectively affects the mode shapes identified by DMD method, especially for Mode 3 and 7. For $\sigma_2=2.5$, the GPR-based modes remain almost the same as the true DMD modes, with some minor changes in modal amplitudes, while for DMD method one can readily observe the strong contribution from the noise mode for every identified modes.

The mode shapes are further compared quantitatively via correlation contour plots in Fig. \ref{fig:gpr_dmd_proj}.  The set of noise-free DMD modes are compared pairwise with the sets of GPR-based modes and noisy DMD modes.  Every two modes, $\vu_i$ and $\vu_j$, are compared by a correlation metric, i.e., the inner product that reveals the angle between the two modes,
\begin{equation}\label{proj}
    \cos \theta = \frac{\vu_i^* \vu_j}{\norm{\vu_i}\norm{\vu_j}}, \quad 0 \leq \cos \theta \leq 1
\end{equation}
Two modes are more similar when $\cos \theta$ is close to 1.  In Fig. \ref{fig:gpr_dmd_proj}, five noise levels are considered, $\sigma_2=0.5, 1.0, 1.5, 2.0, 2.5$.  At the lowest noise level, both correlation contours show a dominantly diagonal pattern, indicating that both GPR modes and noisy DMD modes capture the true DMD modes well.  However, as the noise level increases, the correlation plots for noisy DMD modes quickly smear out, which means the deviation of the modes from the noise-free case.  Meanwhile, the GPR-based results maintained the diagonal structure more robustly throughout all the noise levels.

% The modal comparison can be done by projecting the identified modes to the true DMD modes. This projection is shown in Eq (\ref{proj} where $\boldsymbol{\phi}_i$ corresponds to $i$th DMD mode. We considered 5 different noise level, $\sigma_2=0.5, 1.0, 1.5, 2.0, 2.5$. In Fig. \ref{fig:gpr_dmd_proj}, mode-wise projection is done. First row corresponds to the comparison between DMD without noise and GPR modes, and the second row corresponds to the comparison between DMD without noise and with noise. One can easily notice that as the noise level increases, the diagonal elements which was relatively clear in the case of $\sigma_2=0.5$ gets blurred whereas this trend is mostly maintained in the GPR.

\begin{figure}[H]
\centering
\includegraphics[width=0.6\textwidth]{noise_frequency_plot.png}
\caption{Identified frequencies from DMD and GPR.}\label{fig:dmd_gpr_freq}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=0.9\textwidth]{gp_temporal.png}
\caption{Comparison between temporal dynamics between the true DMD modes and GPR-based DMD modes for $\sigma_2=2.5$}\label{fig:gp_temporal}
\end{figure}

\begin{figure}[H]
\centering
\insertfigs{true_dmd_modes}{0.208}{True DMD modes}
\insertfigs{noisy_gpr_modes}{0.36}{DMD modes by MVGPR}
\insertfigs{noisy_dmd_modes}{0.36}{Noisy DMD modes}
\caption{Comparison of identified mode shapes for noise levels $\sigma_2=0.5$ and $\sigma_2=2.5$.}
\label{fig:dmd_gp_modes}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{GPR_DMD_noise.png}
\caption{Correlation plots between true DMD modes, noisy DMD modes, and GPR-based modes over all noise levels.}\label{fig:gpr_dmd_proj}
\end{figure}


\subsubsection{Sparse Measurement Data}
This test case considers a more challenging scenario for standard DMD techniques, where the dataset is sparse, i.e., the snapshots are non-uniformly distributed.  The sparsity is achieved by randomly removing some of the data points from the original data set.  The percentages of retained data range from 50\% to 20\%.

For the GPR model, 8 cosine kernels are employed and the data is projected to a subspace of 8 POD modes.  In DMD algorithm, it is not possible to directly apply it to this type of data. Therefore, cubic interpolation was used to reconstruct the dynamics on a uniform time grid, so that the conventional DMD algorithm can still be applied.  The GPR and interpolated DMD results are compared with the true DMD modes from full dataset.

First, the identified frequencies from both GPR and DMD are plotted in Fig. \ref{fig:dmd_gpr_sparse_freq}. It is clear that GPR model accurately identifies the frequencies for every percentage considered, while for DMD even 51.34 \% of data points cannot capture the two higher frequencies. As retained data decreases, every identified frequency keeps decreasing, and at 20\%, 3 of them are completely wrong. The error in DMD is attributed to the interpolation procedure that contaminates the frequency components.

Next, the temporal prediction of the GPR model is examined for the case of 50\% data in Fig. \ref{fig:gp_sparse_tp}, where the projected coordinates of the sparse data points are compared with the GPR mean prediction and error bounds.  The first thing to note is that, due to the lack of data points, the projected coordinates now contain multiple frequency components.  Yet, the GPR model is able to capture the temporal dynamics almost exactly with an error bound that is nearly zero over all time.  The near-zero error bound is explained by two factors.  First, no white noise kernel is involved in GP, hence the error bound would be zero at sample points.  Second, the GP assumes a periodic kernel structure and only needs to learn the information of one period from data; in the sparse dataset, while each period only contains a partial set of data points, the combination of data points from different periods is likely to densely cover the one entire period for the learning of the periodic kernels, and thus eliminating the errors over all time.

% When it comes to GPR, the error bound is much thinner than that of DMD. This is because, GPR is good at finding the pattern out of the data which specifically means that unless data is completely periodic, GPR can achieve useful information out of the data. Therefore, the result from GPR consistently provides better result than DMD with cubic interpolation.

Subsequently, the mode shapes from GPR and interpolated DMD are compared in Fig. \ref{fig:dmd_gp_modes_sp}.  Even with only 20\% data, GPR is able to capture well the true DMD modes; some mild distortions exist, but the spatial characteristic lengths in each mode are captured well.  As for the interpolated DMD, the modal distortion soon becomes unacceptable once the data percentage is below 40\%.  Furthermore, due to the incorrectly identified frequencies, it becomes difficult to associate the correct orders for the interpolated DMD modes.

Due to the mixing of the interpolated DMD modes, the comparison between the GPR and DMD modes are quantified using the concept of Grassmannian distance \cite{ye2016schubert,Sadagopan2022}.  Unlike the inner product metric that compares two sets of vectors in a pairwise manner, the Grassmannian distance directly compares the subspaces spanned by two sets of vectors.  Suppose the two sets of $k$ vectors are collected column-wise in two matrices, $\vU_1$ and $\vU_2$, the Grassmannian distance is defined as
\begin{equation}
    d(\vU_1,\vU_2) = \left( \sum_{i=1}^k (\cos^{-1}\sigma_i)^2 \right)^{1/2}
\end{equation}
where $\sigma_i$ are the singular values of $\vU_1^T\vU_2$.  From the definition, the Grassmannian distance can be viewed as the angle between two subspaces.

Figure \ref{fig:gm_dist} shows the Grassmannian distances between identified modes and true DMD modes for a range of retained percentages.  For each percentage, the training datasets are randomly generated from the original dataset for 10 times, and the means and min-max bounds are computed.  Overall, as expected, the distances deviate away from the true DMD for both models as the dataset becomes more sparse.  However, the impact of data sparsity is much more dominant on interpolated DMD than the GPR method, both in terms of the mean and the min-max bounds.  Note that on the sparser end of data, the distance of interpolated DMD reaches $\sim$1.7 rad, which indicates that some identified modes are orthogonal to the true modes and hence totally off.  Furthermore, the wide min-max bounds of interpolated DMD mean that the method is highly sensitive to the choice of data points and vulnerable to missing data.  On the contrary, the GPR model is able to consistently produce relatively accurate modes throughout the retained percentages.  Again, such superiority of GPR is attributed to the inductive bias endowed by the periodic kernel structure, that extracts more dynamical information from the sparse dataset.

% For modal comparison, Grassmannian is used to measure the subspace distance. Fig. \ref{fig:dmd_gp_modes} shows both true and identified mode shapes from multi-variate GPR and DMD with cubic interpolation when using only 20\% of the original data. In this highly sparse data set, DMD with cubic interpolation cannot approximate the true trajectory. Therefore, in the mode shape, it is almost impossible to tell which mode corresponds to which mode in true DMD.
% However, for DMD with interpolation as more data points are removed, the subspace distance quickly grows while for GPR, it only slightly increases.
% The min-max bound is also important to note as this provides the sensitivity of the model to the information of the data. 
% This is because for DMD with cubic interpolation, it is important how the data is distributed. If the data is uniformly distributed, then the interpolation might be able to approximate the original dynamics well, which forms the minimum bound. If the sampling is biased to certain region, then DMD cannot approximate the region where the data is rare. Therefore, this leads to the distortion of the frequency in the data, which forms the maximum bound.


\begin{figure}[H]
\centering
\includegraphics[width=.6\textwidth]{sparse_frequency_plot.png}
\caption{Identified frequencies from DMD and GPR.}\label{fig:dmd_gpr_sparse_freq}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.9\textwidth]{sparse_data_gp_temporal.png}
\caption{POD coordinates identified by GPR (50 \% data points).}\label{fig:gp_sparse_tp}
\end{figure}

% \begin{figure}[H]
% \centering
% \insertfigs{dmd_modes_true}{0.25}{True DMD modes}
% \insertfigs{gp_modes_sparse_data}{0.5}{DMD modes identified by multi-variate GPR}
% \insertfigs{dmd_modes_sparse_data}{0.5}{DMD modes identified by DMD with cubic interpolation}
% \caption{True and identified mode shapes for the first 8 DMD modes using 20\% of the data}
% \label{dmd_gp_modes}
% \end{figure}

\begin{figure}[H]
\centering
\insertfigs{sparse_gpr_modes}{0.5}{Identified modes from GPR.}
\insertfigs{true_dmd_modes_sparse}{0.19}{True DMD modes.}
\insertfigs{sparse_dmd_modes}{0.5}{Identified modes from interpolated DMD.}
\insertfigs{true_dmd_modes_sparse}{0.19}{True DMD modes.}
\caption{Comparison of identified mode shapes for different data sparsity levels.}
\label{fig:dmd_gp_modes_sp}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.6\textwidth]{subspace_distance.png}
\caption{Comparison between true and identified modes using the Grassmannian distance.}\label{fig:gm_dist}
\end{figure}

